On a generalization of the preconditioned Crank-Nicolson Metropolis algorithm

Metropolis algorithms for approximate sampling of probability measures on infinite dimensional Hilbert spaces are considered and a generalization of the preconditioned Crank-Nicolson (pCN) proposal is introduced. The new proposal is able to incorporate information of the measure of interest. A numerical simulation of a Bayesian inverse problem indicates that a Metropolis algorithm with such a proposal performs independent of the state space dimension and the variance of the observational noise. Moreover, a qualitative convergence result is provided by a comparison argument for spectral gaps. In particular, it is shown that the generalization inherits geometric ergodicity from the Metropolis algorithm with pCN proposal.

==> macros.tex <==
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{it}

\DeclareMathOperator{\Div}{\nabla\cdot}
\newcommand{\Grad}{\nabla}
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{it}
\renewcommand{\div}{\mathrm{div\,}}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\cost}{cost}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\dist}{dist}
%
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix} }
\newcommand{\prob}{\boldsymbol {\mathsf P}}
%
\newcommand{\vA}{\mathbf A}
\newcommand{\vB}{\mathbf B}
\newcommand{\vC}{\mathbf C}
\newcommand{\vE}{\mathbf E}
\newcommand{\vF}{\mathbf F}
\newcommand{\vH}{\mathbf H}
\newcommand{\vI}{\mathbf I}
\newcommand{\vK}{\mathbf K}
\newcommand{\vL}{\mathbf L}
\newcommand{\vM}{\mathbf M}
\newcommand{\vO}{\mathbf O}
\newcommand{\vS}{\mathbf S}
\newcommand{\vV}{\mathbf V}
\newcommand{\vX}{\mathbf X}
\newcommand{\vY}{\mathbf Y}
\newcommand{\vZ}{\mathbf Z}
\newcommand{\vXiO}{\mathbf Xi}
%
\newcommand{\va}{\mathbf a}
\newcommand{\vc}{\mathbf c}
\newcommand{\vd}{\mathbf d}
\newcommand{\vf}{\mathbf f}
\newcommand{\vh}{\mathbf h}
\newcommand{\vi}{\mathbf i}
\newcommand{\vj}{\mathbf j}
\newcommand{\vk}{\mathbf k}
\newcommand{\vm}{\mathbf m}
\newcommand{\vn}{\mathbf n}
\newcommand{\vq}{\mathbf q}
\newcommand{\vr}{\mathbf r}
\newcommand{\vs}{\mathbf s}
\newcommand{\vt}{\mathbf t}
\newcommand{\vu}{\mathbf u}
\newcommand{\vv}{\mathbf v}
\newcommand{\vx}{\mathbf x}
\newcommand{\vy}{\mathbf y}
\newcommand{\vz}{\mathbf z}

\newcommand{\valpha}{{\boldsymbol \alpha}}
\newcommand{\vbeta}{{\boldsymbol \beta}}
\newcommand{\vgamma}{{\boldsymbol \gamma}}
\newcommand{\veta}{{\boldsymbol \eta}}
\newcommand{\vnu}{{\boldsymbol \nu}}
\newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vvareps}{\boldsymbol{\varepsilon}}
\newcommand{\vxi}{\boldsymbol{\xi}}
\newcommand{\vXi}{\boldsymbol{\Xi}}
\newcommand{\vGamma}{\boldsymbol{\Gamma}}
%
\newcommand{\vell}{{\boldsymbol \ell}}
%
\newcommand{\Aa}{\vec a}
\newcommand{\Ax}{\vec x}
\newcommand{\Ay}{\vec y}
%
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbE}{\mathbb{E}}
\DeclareMathOperator{\1}{\mathrm{ \mathbf{1}}}

\newcommand{\mc}{\mathcal}
%\renewcommand{\span}{\mathrm{span}}


\DeclareMathOperator{\E}{\boldsymbol{\mathsf  E}}
\DeclareMathOperator{\e}{\mathrm e}
\newcommand{\ev}[1]{ {\boldsymbol{\mathsf  E}} \left[  #1 \right]}
%\newcommand{\ev}[1]{\left\langle #1 \right\rangle}
\newcommand{\ip}[1]{\left( #1 \right)}
\renewcommand{\d}{\mathrm{d}}
\DeclareMathOperator{\Cov}{Cov}
\renewcommand{\Pr}{\mathrm{Pr}}
\DeclareMathOperator{\Var}{Var}
\newcommand{\cov}[1]{\Cov\left(#1\right)}

\theoremstyle{definition}
\newtheorem{defi}{Definition}%[section]
\newtheorem{example}[defi]{Example}
% \newtheoremstyle{remark}{}{}{\rm}{0pt}{\it}{}{}{}
% \theoremstyle{remark}
\newtheorem{remark}[defi]{Remark}
% \theoremstyle{plain}
\newtheorem{propo}[defi]{Proposition}
\newtheorem{theo}[defi]{Theorem}
\newtheorem{lem}[defi]{Lemma}
\newtheorem{cor}[defi]{Corollary}



